WoW -- A System for Self-Service Collaborative Design Workshops

In many working environments, users have to solve complex problems relying on large and multi-source data. Such problems require several experts to collaborate on solving them, or a single analyst to reconcile multiple complementary standpoints. Previous research has shown that wall-sized displays supports different collaboration styles, based most often on abstract tasks as proxies of real work. We present the design and implementation of WoW, short for ``Workspace on Wall'', a multi-user Web-based portal for collaborative meetings and workshops in multi-surface environments. We report on a two-year effort spanning context inquiry studies, system design iterations, development, and real testing rounds targeting design engineers in the tire industry. The pneumatic tires found on the market result from a highly collaborative and iterative development process that reconciles conflicting constraints through a series of product design workshops. WoW was found to be a flexible solution to build multi-view set-ups in a self-service manner and an effective means to access more content at once. Our users also felt more engaged in their collaborative problem-solving work using WoW than in conventional meeting rooms.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );

        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> reviews.tex <==
Reviews for CSCW 2022 (January 2022 round) submission 8000:



----------------------------------------------------------------

1AC review (reviewer 1)

  Confidence Somewhat confident - I have passing knowledge

  (Short) Review This paper contributes a system and a case study of an application for supporting collaboration on wall-sized displays in the context of design engineers working in the tire industry.

    What I like about this paper is that the authors clearly engaged in an actual design setting and considered the needs of people using the system in that practical setting. So from a user-centered design perspective, the authors are practically engaged.

    I am, however, much more concerned about this work when considering it's contributions to the larger literature. Here are a few of the major issues:
    - What is the connection of this work to the larger literature on wall-sized displays and collaboration tools therein? The related work discussion is rather high-level, and the main critique of some of the existing systems is that they are not for "ad-hoc meetings" or not "flexible" enough.

    - Perhaps this point about flexibility is something to build on -- but generally, what is the core design contribution that extends beyond this specific application to the larger discussion on how to design interfaces/systems for collaboratively working on wall-sized displays? What are the insights for design over existing designs? From the solution itself, I didn't see too much... I mean, most of the design characteristics seem very straightforward, and doesn't seem to provide new insights for supporting such collaboration. For instance, is there something unique about the setting and the ways that the engineers needed to work, that suggests something that we should generally consider more when designing interfaces for working in this way?

    As now written, the paper reads like a case study of an application for wall-sized displays to a setting, and less like a research paper that provides generalizable design principles and contributions. The system looks interesting as is but more as a useful work tool than an insightful research contribution. The study itself is rather informal, so it's also unclear how generalizable the insights are.

    I am leaving the recommendation as Major Revision for now, but I am not particularly confident that the authors will be able to make all the changes required within a few short months.

  1AC Recommendation to Editors Major Revision 1AC Meta-Review This paper contributes a system and a case study of an application for supporting collaboration on wall-sized displays in the context of design engineers working in the tire industry.

    While reviewers commented that the system looks interesting and effective, there is significant concern about the novelty of this work in terms of the generalizable research contributions that it makes. After some discussion among the reviewers, we are recommending Major Revisions, but with the understanding that the noted issues may not be addressable over the course of an R&R, as it would require rewriting significant portions of the paper.

    Here is a summary of the key concerns from reviewers:


    - The evaluation of the system does not provide substantial new insights into the design, deployment, or use of collaborative large display environments. The particular design arguments + design implications do not appear to add significantly to the literature.
    - The specific connections and improvements over the larger literature on wall-sized displays and collaboration tools is not clearly established. It is not clear what the gneeralizable insights are. There is insufficient discussion of exactly what novel problems are observed or solved in this context, compared to what appears in previous literature.
    - The main contribution of the paper is to provide details on how a large and multi-device display space can be designed and developed for a real-world work context. As described below, there is insufficient discussion of exactly what novel problems are observed or solved in this context, compared to what appears in previous literature.
    - The concern that the evaluation is mostly focused on usability and as such, does not provide much insight into how or why different aspects of the system were successful or unsuccessful in supporting collaboration.

    Overall, to constitute a research contribution, it is not sufficient for the authors to propose a system for a domain they study; this constitutes a case study or a form of user-centered design, but does not by itself indicate a larger research contribution to the field. Such a contribution may involve the observation of a new (class of problems) previously unaddressed, new design principles + implications for addressing such problems, new system characteristics or architectures that can generalize to address a class of problems extending from but beyond the specific setting, and so on.

    We hope the authors find the reviews helpful in moving this work forward.

----------------------------------------------------------------

Reviewer review (reviewer 2)

  Confidence Very confident - I consider myself an expert in the area Recommendation to 1AC Minor Revision Review In this paper, the authors present "Workspace On Wall" (WoW), a collaborative system to do design meetings on an LHRD with participants either remote or colocated. In the first part, the authors proposed an observation study of the current way of doing meetings in a Tire company. They then presented their system and performed 2 usability studies that showed the high potential of their approach.

    Overall, the paper is well written and tackles a topic quite interesting and timely. The motivation to design such systems is well presented both in the introduction and the observation study in Section 3.

    The related work provides a complete view of the scientific landscape and there is no important missing work, to my knowledge.

    The system is quite advanced and proposes a promising approach to collaborative design meetings, which is the outcome of the study presented in Section 6.

    There are, however, minors issues that should be fixed before the publication of this paper:
    (1) Section 3 presents observations of current meetings done in the company. It is interesting and provides good motivation for the design of the system itself. However, most of the findings can be already found in related work and there are a few redundancies. I think it would be worth reducing this part to keep only new insights, which would then reduce the size of the paper (it is already quite long).
    (2) Due to the COVID crisis, most observations were done on online meetings only. A context in which the use of a wall displays is not really possible, and overall rather different from colocated meeting in general. It can be understood that it was not possible to observe in-person meetings at the time and that most findings could be transferable from one session to the other. But it would be interesting to mention this limitation and explain what could be transferable and what would not be.
    (3) It would be interesting to add concrete details about the meetings observed: Which types of meeting (2 types are presented at the beginning but a figure would be good here)? How many participants on average? How long did they last?
    (4) In the study, the authors reported results about observation, but it is not mentioned in the presentation of the study design. How were the observations done? Only notes were taken or did they use video recording? Any logs used?
    (5) Only the participants of the first session are presented. Are the participants in the second the same?
    (6) In the presentation of the results about teamwork, the authors mentioned that participants asked more questions and overall interacted and communicated more. Is this only based on observation or also on quantitative figures? If it is only based on observation, it would be better to be a bit more cautious and clearly state that this is only suggested by observation and not backed up by statistical tests.

    Overall, I think this paper would be a great contribution for the CSCW and that the issues mentioned in this review are minor and could be fixed in the conference submission cycle, and recommend thus to accept the paper with minor revisions.

----------------------------------------------------------------

Reviewer review (reviewer 3)

  Confidence Very confident - I consider myself an expert in the area Recommendation to 1AC Reject Review Summary of recommendation:

    The submission should not be accepted because it does not provide a clear contribution to CSCW research. Although the system presented in the paper looks like an effective system, there are many examples of similar setups in previous literature. The evaluation of the system does not provide substantial new insights into the design, deployment, or use of collaborative large display environments.

    Summary of paper:

    The paper presents the design, implementation, and evaluation of a multi-display collaboration space that includes wall-sized displays and personal devices such as laptops. The system was designed using contextual inquiry over the course of collaboration with an industrial partner. The system was evaluated in two work sessions with the partner.

    The main contribution of the paper is to provide details on how a large and multi-device display space can be designed and developed for a real-world work context. As described below, there is insufficient discussion of exactly what novel problems are observed or solved in this context, compared to what appears in previous literature.

    There are several problems with the research reported in the submission. First, it does not identify a new research problem that needs to be solved (or an existing problem that has an insufficient solution). For a "real-world system" paper to make a research contribution, it must solve research problem: for example, in understanding how collaboration works in the real world, in identifying a novel design factor for collaboration support, in developing a novel system architecture / interaction technique / visualization / etc., or in understanding how a deployed system performed in a realistic task. The submission does not clearly articulate any problem - it simply states that a system has been developed for the context of large multi-device display environments.

    In addition, the results of the contextual inquiry reported in the paper do not indicate a clear research problem that goes beyond previous work. The "observed challenges" reported in section 3.3 are largely the same as what has been reported in several previous studies of co-present collaboration, and the submission does not provide any specifics of the industrial context that could add new insights to these existing collaboration issues.

    Second, the system itself does not provide an architecture or specific features that are novel enough to stand on their own as a research contribution. The system seems to be well built and well designed from a software perspective (and it is definitely true that systems in this space are complex and difficult to build) but most of the capabilities of the system have been seen in many previous large-screen or multi-display collaboration systems. For example, there are papers that cover all of the "design goals" stated in the paper (such as interacting from any distance, allowing multiple sources of data, or supporting different collaboration styles). The submission references much of the important work in this area - the concern is that the authors do not differentiate what they have done from those previous results. (There are also a few areas of missing references, such as the work of J. Biehl on display management):

    Biehl, J. T., Baker, W. T., Bailey, B. P., Tan, D. S., Inkpen, K. M., & Czerwinski, M. (2008, April). Impromptu: a new interaction framework for supporting collaboration in multiple display environments and its field evaluation for co-located software development. In Proceedings of the SIGCHI conference on human factors in computing systems (pp. 939-948).

    Biehl, J. T., Czerwinski, M., Smith, G., & Robertson, G. G. (2007, April). FASTDash: a visual dashboard for fostering awareness in software teams. In Proceedings of the SIGCHI conference on Human factors in computing systems (pp. 1313-1322).

    Biehl, J. T., & Bailey, B. P. (2004, May). ARIS: an interface for application relocation in an interactive space. In Proceedings of Graphics interface 2004 (pp. 107-116).

    Third, the submission's evaluation primarily acts as a usability study of the system, rather than as a mechanism for examining collaboration issues in light of the specific supports provided by the tool. As a result, the evaluation seems superficial and does not provide much insight into how or why different aspects of the system were successful or unsuccessful in supporting collaboration - that is, insights that could be generalized to other domains or systems. The authors do not make use of their real-world context to provide new understanding that arise from that context; the reported findings are all high-level and could have been observed in almost any work environment.

    Overall, the submission does not provide new knowledge about how collaboration works in a specific real-world context, and does not provide new techniques or understanding about how systems can support that collaboration. Digging deeper into the ways in which the tool is used may still provide value, but the current submission does not make a clear contribution to CSCW research.

----------------------------------------------------------------



End of reviews for CSCW 2022 (January 2022 round) submission 8000
